Driver Routing and Scheduling with Synchronization Constraints

This paper investigates a novel type of driver routing and scheduling problem motivated by a practical application in long-distance bus networks. A key difference from other crew scheduling problems is that drivers can be exchanged between buses at arbitrary intermediate stops en route such that our problem requires additional synchronization constraints. We present a mathematical model for this problem that leverages a time-expanded multi-digraph and derive bounds for the total number of required drivers. Moreover, we develop a destructive-bound-enhanced matheuristic that converges to provably optimal solutions and apply it to a real-world case study for Flixbus, one of Europe's leading coach companies. We demonstrate that our matheuristic outperforms a standalone MIP implementation in terms of solution quality and computational time and reduces the number of required drivers by up to 56% compared to approaches currently used in practice. Our solution approach provides feasible solutions for all instances within seconds and solves instances with up to 390 locations and 70 requests optimally with an average computational time under 210 sec. We further study the impact of driver exchanges on the total driver count and show that allowing for such exchanges leads to average savings of 42.69%.

==> figures/cs_impact_intermediate_stops_rev2.tex <==
\begin{figure}[]
	\begin{floatrow}
		\ffigbox[.5\textwidth]{%
			\includegraphics[width=.45\textwidth]{./figures/savings_DE-IS_all_negative_rev2.pdf}%
		}{%
			\caption{\textcolor{blue}{Impact of intermediate stops (all instances)}}%
			\label{fig:impactISall}%
		}
		\ffigbox[.5\textwidth]{%
			\includegraphics[width=.45\textwidth]{./figures/savings_DE-IS_all_toLB_rev2.pdf}%
		}{%
			\caption{\textcolor{blue}{Impact of intermediate stops (all, LB)}}%
			\label{fig:impactISall_toLB}%
		}
	\end{floatrow}
\end{figure}

